DepthP+P: Metric Accurate Monocular Depth Estimation using Planar and Parallax

Current self-supervised monocular depth estimation methods are mostly based on estimating a rigid-body motion representing camera motion. These methods suffer from the well-known scale ambiguity problem in their predictions. We propose DepthP+P, a method that learns to estimate outputs in metric scale by following the traditional planar parallax paradigm. We first align the two frames using a common ground plane which removes the effect of the rotation component in the camera motion. With two neural networks, we predict the depth and the camera translation, which is easier to predict alone compared to predicting it together with rotation. By assuming a known camera height, we can then calculate the induced 2D image motion of a 3D point and use it for reconstructing the target image in a self-supervised monocular approach. We perform experiments on the KITTI driving dataset and show that the planar parallax approach, which only needs to predict camera translation, can be a metrically accurate alternative to the current methods that rely on estimating 6DoF camera motion.

==> tables/kitti_main_2.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{l | l| c c c c | c c c }
    \toprule
{\multirow{2}{*}{\bf GT}} & {\multirow{2}{*}{\bf Method}} & \multicolumn{4}{c}{Lower Better} & \multicolumn{3}{c}{Higher Better} \tabularnewline 
& & Abs Rel & Sq Rel & RMSE & RMSE$_{log}$ & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < 1.25^3$\tabularnewline \hline
\parbox[t]{0.2mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{\small{Original Ground Truth \cite{Eigen2014NeurIPS}}}}}
%
& Zhou \etal \cite{Zhou2017CVPR} &  0.183 & 1.595 & 6.709 & 0.270 & 0.734 & 0.902 & 0.959 \tabularnewline 
& Yang \etal \cite{Yang2018AAAI} &  0.182 & 1.481 & 6.501 & 0.267 & 0.725 & 0.906 & 0.963 \tabularnewline 
& Mahjourian \etal \cite{Mahjourian2018CVPR} &  0.163 & 1.240 & 6.220 & 0.250 & 0.762 & 0.916 & 0.968 \tabularnewline
& Yin \etal \cite{Yin2018CVPR} &  0.149 & 1.060 & 5.567 & 2.226 & 0.796 & 0.935 & 0.975 \tabularnewline
& Wang \etal \cite{Wang2018CVPR} &  0.151 & 1.257 & 5.583 & 0.228 & 0.810 & 0.936 & 0.974 \tabularnewline
& Zou \etal \cite{Zou2018ECCV} &  0.150 & 1.124 & 5.507 & 0.223 & 0.806 & 0.933 & 0.973 \tabularnewline
& Yang \etal \cite{Yang2018CVPR} &  0.162 & 1.352 & 6.276 & 0.252 & - & - & - \tabularnewline
& Ranjan \etal \cite{Ranjan2019CVPR} &  0.148 & 1.149 & 5.464 & 0.226 & 0.815 & 0.935 & 0.973 \tabularnewline
& Luo \etal \cite{Luo2019PAMI} &  0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976 \tabularnewline
& Chen \etal \cite{Chen2019ICCV} &  0.118 & 0.905 & 5.096 & 0.211 & 0.839 & 0.945 & 0.977 \tabularnewline
& Godard \etal \cite{Godard2019ICCV} &  \textbf{0.110} & 0.831 & \underline{4.642} & \textbf{0.187} & \textbf{0.883} & \textbf{0.962} & \textbf{0.982} \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} &  \underline{0.111} & \textbf{0.785}   & \textbf{4.601} & \underline{0.189} & 0.878 & \underline{0.960} & \textbf{0.982}\tabularnewline 
& Safadoust \etal &  \textbf{0.110} & \underline{0.792} & 4.700 & \underline{0.189} & \underline{0.881} & \underline{0.960} & \textbf{0.982} \tabularnewline
& DepthP+P (Ours) &  0.152 & 1.322 & 6.185 & 0.239 & 0.781 & 0.920 & 0.970 \tabularnewline \cline{2-9}
& Casser \etal \cite{Casser2019AAAI} & 0.141 & 1.026 & 5.291 & 0.215 & 0.816 & 0.945 & 0.979 \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} &  0.111 & 0.829 & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 \tabularnewline
& Guizilini \etal \cite{Guizilini2020ICLR} & 0.102 & 0.698 & 4.381 & 0.178 & 0.896 & 0.964 & 0.984 \tabularnewline \hline\hline 
%\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\small{Improved GT \cite{Uhrig2017THREEDV}}}}} %&
& Zhou \etal \cite{Zhou2017CVPR} &  0.176 & 1.532 & 6.129 & 0.244 & 0.758 & 0.921 & 0.971 \tabularnewline
& Mahjourian \etal \cite{Mahjourian2018CVPR} &  0.134 & 0.983 & 5.501 & 0.203 & 0.827 & 0.944 & 0.981 \tabularnewline
& Yin \etal \cite{Yin2018CVPR} &  0.132 & 0.994 & 5.240 & 0.193 & 0.833 & 0.953 & 0.985 \tabularnewline
& Wang \etal \cite{Wang2018CVPR} &  0.126 & 0.866 & 4.932 & 0.185 & 0.851 & 0.958 & 0.986 \tabularnewline
& Ranjan \etal \cite{Ranjan2019CVPR} &  0.123 & 0.881 & 4.834 & 0.181 & 0.860 & 0.959 & 0.985 \tabularnewline
& Luo \etal \cite{Luo2019PAMI} &  0.120 & 0.789 & 4.755 & 0.177 & 0.856 & 0.961 & 0.987 \tabularnewline
& Godard \etal \cite{Godard2019ICCV} &  \underline{0.085} & 0.468 & \underline{3.672} & \underline{0.128} & \underline{0.921} & \underline{0.985} & \underline{0.995} \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} &  \textbf{0.078} & \textbf{0.420} & \textbf{3.485} & \textbf{0.121} & \textbf{0.931} & \textbf{0.986} & \textbf{0.996} \tabularnewline
& Safadoust \etal  &  \underline{0.085} & \underline{0.458} & 3.779 & 0.131 & 0.919 & \underline{0.985} & \textbf{0.996} \tabularnewline
& DepthP+P (Ours) &  0.134 & 1.042 & 5.566 & 0.199 & 0.820 & 0.946 & 0.983
\end{tabular}

    % \vspace{2pt}
    \caption{\textbf{Quantitative Results for Monocular Training on KITTI.} This table compares our proposed approaches, \textbf{MonoDepthSeg} and \textbf{DepthP+P}, to previous approaches on the KITTI dataset using the original and improved ground truth. 
    %dataset for depth estimations up to 80m. 
    The \textbf{Supervision} column shows different types of supervision used by different methods and \textbf{M} stands for monocular sequences. \textbf{Sem} and \textbf{Ins} refer to using semantic or instance information, respectively. \textbf{v} refers to velocity supervision. We show the results for the input resolution $640 \times 192$. The best self-supervised method in each column is shown in bold and the second best is underlined.}
    \label{tab:kitti_main2}
    % \vspace{-2pt}
\end{table*}

==> tables/kitti_main_3.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{l | l | c | c c c c | c c c }
    \toprule
& {\multirow{2}{*}{\bf Method}} & {\multirow{2}{*}{\bf Supervision}} & \multicolumn{4}{c}{Lower Better} & \multicolumn{3}{c}{Higher Better} \tabularnewline 
& & & Abs Rel & Sq Rel & RMSE & RMSE$_{log}$ & $\delta < 1.25$ & $\delta < 1.25^2$ & $\delta < 1.25^3$\tabularnewline \hline
\parbox[t]{2mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{\small{Original Ground Truth \cite{Eigen2014NeurIPS}}}}}
%
& Zhou \etal \cite{Zhou2017CVPR} & M & 0.183 & 1.595 & 6.709 & 0.270 & 0.734 & 0.902 & 0.959 \tabularnewline 
& Yang \etal \cite{Yang2018AAAI} & M & 0.182 & 1.481 & 6.501 & 0.267 & 0.725 & 0.906 & 0.963 \tabularnewline 
& Mahjourian \etal \cite{Mahjourian2018CVPR} & M & 0.163 & 1.240 & 6.220 & 0.250 & 0.762 & 0.916 & 0.968 \tabularnewline
& Yin \etal \cite{Yin2018CVPR} & M & 0.149 & 1.060 & 5.567 & 2.226 & 0.796 & 0.935 & 0.975 \tabularnewline
& Wang \etal \cite{Wang2018CVPR} & M & 0.151 & 1.257 & 5.583 & 0.228 & 0.810 & 0.936 & 0.974 \tabularnewline
& Zou \etal \cite{Zou2018ECCV} & M & 0.150 & 1.124 & 5.507 & 0.223 & 0.806 & 0.933 & 0.973 \tabularnewline
& Yang \etal \cite{Yang2018CVPR} & M & 0.162 & 1.352 & 6.276 & 0.252 & - & - & - \tabularnewline
& Ranjan \etal \cite{Ranjan2019CVPR} & M & 0.148 & 1.149 & 5.464 & 0.226 & 0.815 & 0.935 & 0.973 \tabularnewline
& Luo \etal \cite{Luo2019PAMI} & M & 0.141 & 1.029 & 5.350 & 0.216 & 0.816 & 0.941 & 0.976 \tabularnewline
& Chen \etal \cite{Chen2019ICCV} & M & 0.118 & 0.905 & 5.096 & 0.211 & 0.839 & 0.945 & 0.977 \tabularnewline
& Godard \etal \cite{Godard2019ICCV} & M & \textbf{0.110} & 0.831 & \underline{4.642} & \textbf{0.187} & \textbf{0.883} & \textbf{0.962} & \textbf{0.982} \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} & M & \underline{0.111} & \textbf{0.785}   & \textbf{4.601} & \underline{0.189} & 0.878 & \underline{0.960} & \textbf{0.982}\tabularnewline 
& Safadoust \etal & M & \textbf{0.110} & \underline{0.792} & 4.700 & \underline{0.189} & \underline{0.881} & \underline{0.960} & \textbf{0.982} \tabularnewline
& DepthP+P (Ours) & M & 0.152 & 1.322 & 6.185 & 0.239 & 0.781 & 0.920 & 0.970 \tabularnewline \cline{2-10}
& Casser \etal \cite{Casser2019AAAI} & M+Ins & 0.141 & 1.026 & 5.291 & 0.215 & 0.816 & 0.945 & 0.979 \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} & M+v & 0.111 & 0.829 & 4.788 & 0.199 & 0.864 & 0.954 & 0.980 \tabularnewline
& Guizilini \etal \cite{Guizilini2020ICLR} & M+Sem & 0.102 & 0.698 & 4.381 & 0.178 & 0.896 & 0.964 & 0.984 \tabularnewline \hline\hline 
%\midrule
\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\small{Improved GT \cite{Uhrig2017THREEDV}}}}} %&
& Zhou \etal \cite{Zhou2017CVPR} & M & 0.176 & 1.532 & 6.129 & 0.244 & 0.758 & 0.921 & 0.971 \tabularnewline
& Mahjourian \etal \cite{Mahjourian2018CVPR} & M & 0.134 & 0.983 & 5.501 & 0.203 & 0.827 & 0.944 & 0.981 \tabularnewline
& Yin \etal \cite{Yin2018CVPR} & M & 0.132 & 0.994 & 5.240 & 0.193 & 0.833 & 0.953 & 0.985 \tabularnewline
& Wang \etal \cite{Wang2018CVPR} & M & 0.126 & 0.866 & 4.932 & 0.185 & 0.851 & 0.958 & 0.986 \tabularnewline
& Ranjan \etal \cite{Ranjan2019CVPR} & M & 0.123 & 0.881 & 4.834 & 0.181 & 0.860 & 0.959 & 0.985 \tabularnewline
& Luo \etal \cite{Luo2019PAMI} & M & 0.120 & 0.789 & 4.755 & 0.177 & 0.856 & 0.961 & 0.987 \tabularnewline
& Godard \etal \cite{Godard2019ICCV} & M & \underline{0.085} & 0.468 & \underline{3.672} & \underline{0.128} & \underline{0.921} & \underline{0.985} & \underline{0.995} \tabularnewline
& Guizilini \etal \cite{Guizilini2020CVPR} & M & \textbf{0.078} & \textbf{0.420} & \textbf{3.485} & \textbf{0.121} & \textbf{0.931} & \textbf{0.986} & \textbf{0.996} \tabularnewline
& Safadoust \etal  & M & \underline{0.085} & \underline{0.458} & 3.779 & 0.131 & 0.919 & \underline{0.985} & \textbf{0.996} \tabularnewline
& DepthP+P (Ours) & M & 0.134 & 1.042 & 5.566 & 0.199 & 0.820 & 0.946 & 0.983
\end{tabular}
\end{adjustbox}
    % \vspace{2pt}
    \caption{\textbf{Quantitative Results for Monocular Training on KITTI.} This table compares our proposed \textbf{DepthP+P} approach to previous approaches on the KITTI dataset using the original and improved ground truth. 
    %dataset for depth estimations up to 80m. 
    The \textbf{Supervision} column shows different types of supervision used by different methods and \textbf{M} stands for monocular sequences. \textbf{Sem} and \textbf{Ins} refer to using semantic or instance information, respectively. \textbf{v} refers to velocity supervision. We show the results for the input resolution $640 \times 192$. The best self-supervised method in each column is shown in bold and the second best is underlined.}
    \label{tab:kitti_main_3}
    % \vspace{-2pt}
\end{table*}
